InfoClus: Informative Clustering of High-dimensional Data Embeddings

Developing an understanding of high-dimensional data can be facilitated by visualizing that data using dimensionality reduction. However, the low-dimensional embeddings are often difficult to interpret. To facilitate the exploration and interpretation of low-dimensional embeddings, we introduce a new concept named partitioning with explanations. The idea is to partition the data shown through the embedding into groups, each of which is given a sparse explanation using the original high-dimensional attributes. We introduce an objective function that quantifies how much we can learn through observing the explanations of the data partitioning, using information theory, and also how complex the explanations are. Through parameterization of the complexity, we can tune the solutions towards the desired granularity. We propose InfoClus, which optimizes the partitioning and explanations jointly, through greedy search constrained over a hierarchical clustering. We conduct a qualitative and quantitative analysis of InfoClus on three data sets. We contrast the results on the Cytometry data with published manual analysis results, and compare with two other recent methods for explaining embeddings (RVX and VERA). These comparisons highlight that InfoClus has distinct advantages over existing procedures and methods. We find that InfoClus can automatically create good starting points for the analysis of dimensionality-reduction-based scatter plots.

==> Notes/2025-03-03.tex <==
Experiments

Separated into:
Case study - i/ three datasets (introduced) + case studies; ii/ hyperparameters; iii/ scalability

This week
Methodology: illustrated with a 4-point, 2-d example 
Jef: looked at paper again; inserted comments
Create entry in the ECML-PKDD website
(Abstract: required by end of week)

In experiments: often, word "clustering" used. Rather: use a PwX when relevant, but clustering is fine

Introduction -> comment wrt Figure 1. The tree in the intro is not necessary at the introduction-level. (Figure wrt splitting still welcome in Section 3)

Open question: what is InfoClus? Both k-means and hierarchical

G\&F: Write method and and experiment section together

Scalability analysis

Per iteration -> trend not clear
Per clustering: make more clear what is meant by this line, maybe clear this up by mentioning pseudo code
t-sne in setup or not?

experiments: mention machine used

Experiments complete?
Yes, but small points might be changed

Goal: full draft by the end of the week (Maarten?)


==> Notes/2025-03-11.tex <==
explanation: distribution? attribute? statistics?
-> += *and their corresponding distribution*

3.1
Move def 2.1 (PwX) to intro
